On finding short reconfiguration sequences between independent sets

Assume we are given a graph $G$, two independent sets $S$ and $T$ in $G$ of size $k \geq 1$, and a positive integer $\ell \geq 1$. The goal is to decide whether there exists a sequence $\langle I_0, I_1, ..., I_\ell \rangle$ of independent sets such that for all $j \in \{0,\ldots,\ell-1\}$ the set $I_j$ is an independent set of size $k$, $I_0 = S$, $I_\ell = T$, and $I_{j+1}$ is obtained from $I_j$ by a predetermined reconfiguration rule. We consider two reconfiguration rules. Intuitively, we view each independent set as a collection of tokens placed on the vertices of the graph. Then, the Token Sliding Optimization (TSO) problem asks whether there exists a sequence of at most $\ell$ steps that transforms $S$ into $T$, where at each step we are allowed to slide one token from a vertex to an unoccupied neighboring vertex. In the Token Jumping Optimization (TJO) problem, at each step, we are allowed to jump one token from a vertex to any other unoccupied vertex of the graph. Both TSO and TJO are known to be fixed-parameter tractable when parameterized by $\ell$ on nowhere dense classes of graphs. In this work, we show that both problems are fixed-parameter tractable for parameter $k + \ell + d$ on $d$-degenerate graphs as well as for parameter $|M| + \ell + \Delta$ on graphs having a modulator $M$ whose deletion leaves a graph of maximum degree $\Delta$. We complement these result by showing that for parameter $\ell$ alone both problems become W[1]-hard already on $2$-degenerate graphs. Our positive result makes use of the notion of independence covering families introduced by Lokshtanov et al. Finally, we show that using such families one can obtain a simpler and unified algorithm for the standard Token Jumping Reachability problem parameterized by $k$ on both degenerate and nowhere dense classes of graphs.

==> conclusion.tex <==

\section{Conclusion}\label{sec:conclusion}

Can we show that token sliding param by $k$ is FPT on degenerate graphs by using sunflowers and studying the neighborhood of a sunflower? 
Can we bound the behavior of vertices having high degree into the sunflower? Can we bound the number of vertices inside the sunflower that have large degree into other petals?
After having done all that can we reduce the number of petals in the sunflower?

==> preamble.tex <==
%generic%%%
\usepackage{amsfonts,amsthm,amsmath}
\usepackage{amstext}
\usepackage{wasysym}
\usepackage{bm}

%%%pagewise footnote numbering%%%
\makeatletter
\@addtoreset{footnote}{section}
\makeatother
%%%%%%%%%%%

\usepackage{tikz}
\usepackage{thm-restate}

\usetikzlibrary{shapes.geometric,matrix,shapes,arrows,positioning,chains}
\usepackage[normalem]{ulem}
\newcommand{\longversion}[1]{#1}
\newcommand{\shortversion}[1]{}
\newcommand{\bigoh}{{\mathcal{O}}}
\usepackage{todonotes}
\usepackage{graphicx,tikz}
\RequirePackage{fancyhdr}
\usepackage{xcolor}
\usepackage{boxedminipage}
\usepackage[ruled,vlined,linesnumbered]{algorithm2e}
\usepackage{stmaryrd,bbm}

\newcommand{\myparagraph}[1]{\smallskip\noindent{\textbf{\sffamily #1} \ }}
\newcommand{\mypara}[1]{\smallskip\noindent{\textbf{\sffamily #1} \ }}

%%complexity classes%%%
\newcommand{\NP}{\textsf{NP}}
\newcommand{\NPp}{${\sf NP}$}
\newcommand{\classP}{\textsf{P}}
\newcommand{\APX}{\textsf{APX}}
\newcommand{\FPT}{{\rm \textsf{FPT}}}
\newcommand{\coNP}{\text{\normalfont co-NP}}
\newcommand{\XP}{\text{\normalfont XP}}
\newcommand{\W}[1][xxxx]{\text{\normalfont W[#1]}}
\newcommand{\WOH}{\textsf{W[1]}-hard}
\newcommand{\WTH}{\textsf{W[2]}-hard}
\newcommand{\WTC}{\textsf{W[2]}-complete}
\newcommand{\NPH}{\textsf{NP}-hard}
\newcommand{\NPC}{\textsf{NP}-complete}
%%%%

%%problem definition box

\newcommand{\defparproblem}[4]{
  \vspace{1mm}
\noindent\fbox{
  \begin{minipage}{0.96\textwidth}
  \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lr} #1  & {\bf{Parameter:}} #3 \\ \end{tabular*}
  {\bf{Input:}} #2  \\
  {\bf{Question:}} #4
  \end{minipage}
  }
  \vspace{1mm}
}

\newcommand{\defproblem}[3]{
  \vspace{1mm}
\noindent\fbox{
  \begin{minipage}{0.96\textwidth}
  \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lr} #1 \\ \end{tabular*}
  {\bf{Input:}} #2  \\
  {\bf{Question:}} #3
  \end{minipage}
  }
  \vspace{1mm}
}

%%

%%useful math macros%
\newcommand{\C}[1]{\mathcal{#1}}
\newcommand{\SC}[1]{\mathscr{#1}}
\newcommand{\BB}[1]{\mathbb{#1}}
\newcommand{\what}{\widehat}
\newcommand{\wtilde}{\widetilde}
%%%%%%%%%%%%%%%%%%%%%

%%%generic fpt paper macros%

%\newtheorem*{theorem*}{Theorem}
%\newtheorem{theorem}{Theorem}
%\newtheorem{lemma}{Lemma}[section]
%\newtheorem{claim}{Claim}[section]
%\newtheorem{corollary}{Corollary}
%\newtheorem{definition}{Definition}[section]
%\newtheorem{observation}{Observation}[section]
%\newtheorem{proposition}{Proposition}[section]
\newcounter{reduction}
\setcounter{reduction}{0}

\newcounter{markingrule}
\setcounter{markingrule}{0}

\newtheorem{mschm}[markingrule]{Marking Scheme}
\newtheorem{redr}[reduction]{Reduction Rule}
\newtheorem{marule}[markingrule]{Marking Rule}

\newcounter{hypothesis}
\setcounter{hypothesis}{0}

\newtheorem{hypo}[hypothesis]{Conjecture}

\newcommand{\Yes}{\textsf{yes}}
\newcommand{\No}{\textsf{no}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Paper specific macros%

\newcommand{\BTJ}{\textsc{Bipartite Token Jumping}}
\newcommand{\Biclique}{\textsc{Bi-clique}}
\newcommand{\MBB}{\textsc{Maximum Balanced Biclique}}
\newcommand{\optbiclq}{{\sf opt}\mbox{-}{\sf biclq}}
\newcommand{\TSAT}{\textsc{$3$-SAT}}
\newcommand{\TD}{\textsc{Skew Detection}} 
\newcommand{\BTS}{\textsc{Bipartite Skew Subgraph}}
\newcommand{\BTIS}{\textsc{Bipartite Skew Induced-Subgraph}}
\newcommand{\BTCS}{\textsc{Bipartite Skew (Induced-)Subgraph}}
\newcommand{\TJ}{\textsc{Token Jumping}} 
%%%%%%%%%%%%%%%%%%%%%%%%

